Agents Thinking Fast and Slow: A Talker-Reasoner Architecture

Large language models have enabled agents of all kinds to interact with users through natural conversation. Consequently, agents now have two jobs: conversing and planning/reasoning. Their conversational responses must be informed by all available information, and their actions must help to achieve goals. This dichotomy between conversing with the user and doing multi-step reasoning and planning can be seen as analogous to the human systems of "thinking fast and slow" as introduced by Kahneman. Our approach is comprised of a "Talker" agent (System 1) that is fast and intuitive, and tasked with synthesizing the conversational response; and a "Reasoner" agent (System 2) that is slower, more deliberative, and more logical, and is tasked with multi-step reasoning and planning, calling tools, performing actions in the world, and thereby producing the new agent state. We describe the new Talker-Reasoner architecture and discuss its advantages, including modularity and decreased latency. We ground the discussion in the context of a sleep coaching agent, in order to demonstrate real-world relevance.

==> methods.tex <==

\noindent \textbf{POMDP Setup.}

\noindent \textbf{}


\noindent \textbf{Formalizing the Reasoner as a POMDP.} At every point in time the Reasoner can make decisions and devise plans given partial information about the world. Specifically, the Reasoner forms beliefs about the world. In our setting, we can assume that the world and the environment are the same, and they are both realized by the user interacting with the conversational system. As a partially observable setting, the thinking slow process of the Reasoner can be formulated as a POMDP. At timestep $t$, the environment is in state $s_t$; but the reasoner can only form its probabilistic belief about the state $b_t$, and thus can learn policy $\pi(a_t | b_t)$ mapping belief $b_t$ to action $a_t$. After executing its action, the environment transitions to $s_{t+1}$ and the reasoner observes $o_{t+1}$, a function of the new state that is used to update the belief state.       

\noindent \textbf{Learning belief states of the world via LLMs.} %Let's delve deeper into how the Reasoner forms beliefs about the world and what these beliefs represent as well as all the thinking slow process incurring from timestep $t$ to $t+1$. 
The belief state represents all the Reasoner knows/believes about the world at a given point in time. This is realized by a structured object (e.g., JSON or XML) with different fields; in the context of a life coaching agent we developed, those fields include the user's goals, barriers, habits, and any potential plan that the agent has given to the user. Every time the Reasoner updates its belief state, the belief state is stored in the memory component. Updating the beliefs is realized via LLM in-context learning. Therefore, the belief state therefore in some sense represents an estimate of the world model of the user, including the user's goals and beliefs, but instead of estimating the user's plan, the Reasoner provides a plan to the user. 

\noindent \textbf{Reasoner as a ReAct-Extract Agent.} From time $t$ to $t+1$ the Reasoner can perform multi-step reasoning and planning. To achieve that, we augment the action space $\mathcal{A}$ to $\hat{\mathcal{A}}$ where $\hat{\mathcal{A}} = \mathcal{A} \cup \mathcal{T} \cup \matchal{E}$ with $\mathcal{T}$ denoting thoughts and $\mathcal{E}$ denoting the constrained decoding extractions. The Reasoner can think, act, and extract to the right schemas. This can be seen as an augmentation of the ReAct framework into a ReAct-Extract framework. The extract action, which can be thought of as structured reasoning, allows for updating the belief state across the reasoning traces. Thus, the belief state $b_{t+1}$ is a result of interleaving among potentially many thoughts $t$ (reasoning), mini-actions $a$ (e.g., calling tools like \texttt{SEARCH}), observations after these actions (e.g., results from search), and extractions $e$ into constrained decoding. 

\noindent \textbf{Reasoner as a hierarchical agent invoking mini-Reasoners.} So far we have assumed that the Reasoner is a single agent performing a series of actions, thoughts, and extractions that lead to the update of the belief state. However, in our approach, it is a hierarchical agent that first updates its belief about parts of the world (e.g., what the user needs help with, understanding the user?), and then given this macro-action invokes the appropriate sub-agent. Depending on the complexity of the task, sub-agents may act, extract, plan, or perform combinations of those steps until a plan is constructed. The planner agent itself can be hierarchical first decomposing the problem into sub-steps and then solving (thinking, acting, extracting) each sub-step.   

\noindent \textbf{Talker interacting with the world/environment/user.} 
The Talker interacts with the world and obtains observations that are then passed to the Reasoner, which updates its beliefs about the world. The Talker can be a standard in-context learned foundational model that takes as input the previous belief state $b_{t}$ and the previous observation $o_t$ to generate its conversational response $c_t$. In this way, the action of the Talker is $r_t$ can completely ignore the Reasoner's belief state if it is not updated, or can update the structured object of belief state to a conversational format adhering to the Talker's instructions. Those instructions can vary based on a part of the belief state.

\noindent \textbf{Updating beliefs based on natural language rewards/Feedback.} The user's linguistic responds to the Talker agent ($c_t$) forms the observation $o_t$ or reward $r_t$. In the life coach agent context, the user might provide further context, or explicit feedback on whether they liked what the Talker agent said previously. We treat observation $o_t$ and $r_t$ which is associated with the talker agent's response $c_t$ for user's / world's state $s_t$. Where notably the $c_t$ is a function of the reasoner's state $b_t$. This feedback then in natural language format will be stored in memory, and will be passed to the reasoner agent to update its beliefs about the world $b_(t+1) \sim \texttt{Reasoner} (\hat{a} | b_t; \Theta) $ where $\Theta$ represent all the parameters of the Reasoner model. This will in turn lead to interactive planning. \kc{delve deeper into interactive planning.}

\noindent \textbf{Reasoner-Talker Updates.}
The Reasoner-Talked architecture updates as follows:  
\begin{equation}
    b_{(t+1)}, a_{(t+1)} \sim \texttt{Reasoner} (b, \hat{a} | b_t, r_t; \Theta) 
\end{equation} (\kc{or could we have belief encompass both the action and the belief?})

\begin{equation}
    c_{(t+1)} \sim \texttt{Talker} (c | b_{(t+1)}, r_t; \Phi) 
\end{equation} where $\Phi$ are the parameters of the Talker.

The above formalization assumes that the Talker waits for the Reasoner to finish its thinking slow process. In practice, to decouple the two and to minimize latency, instead of $b_{(t+1)}$ the Talker uses the latest available belief state $b$ stored in memory. This is effective for tasks that do not require the Reasoner and where the Talker is sufficient. However, there are cases where the reasoner must update its belief state before the Talker proceeds; this is crucial for complex problem-solving scenarios such as when the user is asking for an explicit multi-step plan, or for specific resources that would only result from tool call scenarios such as numerical reasoning.




==> state_formulation.tex <==
%Let's consider the setting of developing a personalized agent to help with some long-term task. We take a reinforcement learning view of the problem \cite{}. The agent is responsible for generating the next agent state $s$ and providing a conversational response $r$. Typically the response is a function of the agent state.  Learn the state via a series of calls to foundational models (LLMs) and tool use and other expert models. Instantiating the world model as an LLM. Model-based RL? Can we assume that what the user says is also textual feedback that then allows us to alter the policy / plan? We need to talk about conversation history as opposed to memory and as opposed to state.========================


\kc{The main thing I haven't talked about yet is the hierarchical planning. I should talk about it in the Reasoner to say that the mini-reasoners update the different parts of the state. And to also say about . Also Reasoner is really interleaving tools and reasoning, both CoT and ReAct}


\noindent \textbf{Formalizing the Reasoner as a POMDP.} At every point in time the Reasoner can make decisions and devise plans given partial information about the world. Specifically, the Reasoner forms beliefs about the world. In our setting, we can assume that the world and the environment are the same, and they are both realized by the user interacting with the conversational system. As a partially observable setting, the thinking slow process of the Reasoner can be formulated as a POMDP. At timestep $t$, the environment is in state $s_t$; but the reasoner can only form its probabilistic belief about the state $b_t$, and thus can learn policy $\pi(a_t | b_t)$ mapping belief $b_t$ to action $a_t$. After executing its action, the environment transitions to $s_{t+1}$ and the reasoner observes $o_{t+1}$, a function of the new state that is used to update the belief state.       

\noindent \textbf{Learning belief states of the world via LLMs.} %Let's delve deeper into how the Reasoner forms beliefs about the world and what these beliefs represent as well as all the thinking slow process incurring from timestep $t$ to $t+1$. 
The belief state represents all the Reasoner knows/believes about the world at a given point in time. This is realized by a structured object (e.g., JSON or XML) with different fields; in the context of a life coaching agent we developed, those fields include the user's goals, barriers, habits, and any potential plan that the agent has given to the user. Every time the Reasoner updates its belief state, the belief state is stored in the memory component. Updating the beliefs is realized via LLM in-context learning. Therefore, the belief state therefore in some sense represents an estimate of the world model of the user, including the user's goals and beliefs, but instead of estimating the user's plan, the Reasoner provides a plan to the user. 

\noindent \textbf{Reasoner as a ReAct-Extract Agent.} From time $t$ to $t+1$ the Reasoner can perform multi-step reasoning and planning. To achieve that, we augment the action space $\mathcal{A}$ to $\hat{\mathcal{A}}$ where $\hat{\mathcal{A}} = \mathcal{A} \cup \mathcal{T} \cup \matchal{E}$ with $\mathcal{T}$ denoting thoughts and $\mathcal{E}$ denoting the constrained decoding extractions. The Reasoner can think, act, and extract to the right schemas. This can be seen as an augmentation of the ReAct framework into a ReAct-Extract framework. The extract action, which can be thought of as structured reasoning, allows for updating the belief state across the reasoning traces. Thus, the belief state $b_{t+1}$ is a result of interleaving among potentially many thoughts $t$ (reasoning), mini-actions $a$ (e.g., calling tools like \texttt{SEARCH}), observations after these actions (e.g., results from search), and extractions $e$ into constrained decoding. 

\noindent \textbf{Reasoner as a hierarchical agent invoking mini-Reasoners.} So far we have assumed that the Reasoner is a single agent performing a series of actions, thoughts, and extractions that lead to the update of the belief state. However, in our approach, it is a hierarchical agent that first updates its belief about parts of the world (e.g., what the user needs help with, understanding the user?), and then given this macro-action invokes the appropriate sub-agent. Depending on the complexity of the task, sub-agents may act, extract, plan, or perform combinations of those steps until a plan is constructed. The planner agent itself can be hierarchical first decomposing the problem into sub-steps and then solving (thinking, acting, extracting) each sub-step.   

\noindent \textbf{Talker interacting with the world/environment/user.} 
The Talker interacts with the world and obtains observations that are then passed to the Reasoner, which updates its beliefs about the world. The Talker can be a standard in-context learned foundational model that takes as input the previous belief state $b_{t}$ and the previous observation $o_t$ to generate its conversational response $c_t$. In this way, the action of the Talker is $r_t$ can completely ignore the Reasoner's belief state if it is not updated, or can update the structured object of belief state to a conversational format adhering to the Talker's instructions. Those instructions can vary based on a part of the belief state.

\noindent \textbf{Updating beliefs based on natural language rewards/Feedback.} The user's linguistic responds to the Talker agent ($c_t$) forms the observation $o_t$ or reward $r_t$. In the life coach agent context, the user might provide further context, or explicit feedback on whether they liked what the Talker agent said previously. We treat observation $o_t$ and $r_t$ which is associated with the talker agent's response $c_t$ for user's / world's state $s_t$. Where notably the $c_t$ is a function of the reasoner's state $b_t$. This feedback then in natural language format will be stored in memory, and will be passed to the reasoner agent to update its beliefs about the world $b_(t+1) \sim \texttt{Reasoner} (\hat{a} | b_t; \Theta) $ where $\Theta$ represent all the parameters of the Reasoner model. This will in turn lead to interactive planning. \kc{delve deeper into interactive planning.}

\noindent \textbf{Reasoner-Talker Updates.}
The Reasoner-Talked architecture updates as follows:  
\begin{equation}
    b_{(t+1)}, a_{(t+1)} \sim \texttt{Reasoner} (b, \hat{a} | b_t, r_t; \Theta) 
\end{equation} (\kc{or could we have belief encompass both the action and the belief?})

\begin{equation}
    c_{(t+1)} \sim \texttt{Talker} (c | b_{(t+1)}, r_t; \Phi) 
\end{equation} where $\Phi$ are the parameters of the Talker.




\kc{finish up connection with theory of mind --> write section 2.3 where we merge info from section 3 to the different parts of 2.3. Mention the actions of Reason, Act, Talk, and Extract. Then describe LLM as Talker. LLM as Reasoner. LLM as Belief State etc.}

\kc{
\begin{itemize}
    \item a lot of the literature doesn't talk about this paradigm of talking to the user and acting at the same time. i don't know if we call that embodiement.
    \item need to talk about state extraction via LLMs and connect that to world models
    \item need to talk about decomposing a problem to sub-problems and doing tool use for each. So need to talk about hierarchical planning
    \item --> see setup for react 
--> focus more on llm-based agents.
--> then say how to decompose into the two systems.
--> for the reasoner i need to decouple LLM as state producer, LLM as planner.
--> for the talker I need to talk about updating based on feedback. and priming based on memory
--> for both i need to say that we do in-context learning, but approaches like verbal feedback etc. could be possible.
\end{itemize}
}
